Gluing theory for slc surfaces and threefolds in positive characteristic

We develop a gluing theory in the sense of Koll\'{a}r for slc surfaces and threefolds in positive characteristic. For surfaces we are able to deal with every positive characteristic $p$, while for threefolds we assume that $p>5$. Along the way we study nodes in characteristic $2$ and establish a theory of sources and springs \`a la Koll\'{a}r for threefolds. We also give applications to the topology of lc centers on slc threefolds, and to the projectivity of the moduli space of stable surfaces in characteristic $p>5$.

==> Macros.tex <==
%\documentclass[a4paper,11pt]{article}
\usepackage[left=1.02in,top=1.0in,right=1.02in,bottom=1.0in]{geometry}
\usepackage{environ}
\usepackage{mabliautoref}
\usepackage{amssymb,amsthm,amsmath}
\RequirePackage[dvipsnames,usenames]{xcolor}
%\usepackage{ifpdf}
\usepackage{hyperref}
\usepackage{mathtools}
%\usepackage[left=1.02in,top=1.0in,right=1.02in,bottom=1.0in]{geometry}
\usepackage[all]{xy}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{enumitem}
%\usepackage{chngcntr}
\usepackage{stmaryrd}
%\usepackage[T1]{fontenc}
%\usepackage{newtxtext,newtxmath}
\usepackage{xfrac}
\usepackage{fix-cm}
\usepackage{faktor}
\usepackage{minibox}


\hypersetup{
bookmarks,
bookmarksdepth=3,
bookmarksopen,
bookmarksnumbered,
pdfstartview=FitH,
colorlinks,backref,hyperindex,
linkcolor=Sepia,
anchorcolor=BurntOrange,
citecolor=MidnightBlue,
citecolor=OliveGreen,
filecolor=BlueViolet,
menucolor=Yellow,
urlcolor=OliveGreen
}

\newcommand{\expl}[2]{\underset{\mathclap{\minibox[c]{$\uparrow$\\ \fbox{\footnotesize #2}}}}{#1}}

\newcommand{\explshift}[3]{\underset{\mathclap{\minibox[c]{$\uparrow$\\ \hspace{#1} \fbox{\footnotesize #3}}}}{#2}}

\newcommand{\explpar}[3]{\underset{\mathclap{\minibox[c]{$\uparrow$\\  \fbox{\parbox{#1}{\footnotesize #3}}}}}{#2}}

\newcommand{\explparshift}[4]{\underset{\mathclap{\minibox[c]{$\uparrow$\\ \hspace{#2} \fbox{\parbox{#1}{\footnotesize #4}}}}}{#3}}



\DeclareMathAlphabet{\mathchanc}{OT1}{pzc}%
                                 {m}{it}

% chancery font
% upper case
\newcommand{\mcA}{\mathchanc{A}}
\newcommand{\mcB}{\mathchanc{B}}
\newcommand{\mcC}{\mathchanc{C}}
\newcommand{\mcD}{\mathchanc{D}}
\newcommand{\mcE}{\mathchanc{E}}
\newcommand{\mcF}{\mathchanc{F}}
\newcommand{\mcG}{\mathchanc{G}}
\newcommand{\mcH}{\mathchanc{H}}
\newcommand{\mcI}{\mathchanc{I}}
\newcommand{\mcJ}{\mathchanc{J}}
\newcommand{\mcK}{\mathchanc{K}}
\newcommand{\mcL}{\mathchanc{L}}
\newcommand{\mcM}{\mathchanc{M}}
\newcommand{\mcN}{\mathchanc{N}}
\newcommand{\mcO}{\mathchanc{O}}
\newcommand{\mcP}{\mathchanc{P}}
\newcommand{\mcQ}{\mathchanc{Q}}
\newcommand{\mcR}{\mathchanc{R}}
\newcommand{\mcS}{\mathchanc{S}}
\newcommand{\mcT}{\mathchanc{T}}
\newcommand{\mcU}{\mathchanc{U}}
\newcommand{\mcV}{\mathchanc{V}}
\newcommand{\mcW}{\mathchanc{W}}
\newcommand{\mcX}{\mathchanc{X}}
\newcommand{\mcY}{\mathchanc{Y}}
\newcommand{\mcZ}{\mathchanc{Z}}
% lower case
\newcommand{\mca}{\mathchanc{a}}
\newcommand{\mcb}{\mathchanc{b}}
\newcommand{\mcc}{\mathchanc{c}}
\newcommand{\mcd}{\mathchanc{d}}
\newcommand{\mce}{\mathchanc{e}}
\newcommand{\mcf}{\mathchanc{f}}
\newcommand{\mcg}{\mathchanc{g}}
\newcommand{\mch}{\mathchanc{h}}
\newcommand{\mci}{\mathchanc{i}}
\newcommand{\mcj}{\mathchanc{j}}
\newcommand{\mck}{\mathchanc{k}}
\newcommand{\mcl}{\mathchanc{l}}
\newcommand{\mcm}{\mathchanc{m}}
\newcommand{\mcn}{\mathchanc{n}}
\newcommand{\mco}{\mathchanc{o}}
\newcommand{\mcp}{\mathchanc{p}}
\newcommand{\mcq}{\mathchanc{q}}
\newcommand{\mcr}{\mathchanc{r}}
\newcommand{\mcs}{\mathchanc{s}}
\newcommand{\mct}{\mathchanc{t}}
\newcommand{\mcu}{\mathchanc{u}}
\newcommand{\mcv}{\mathchanc{v}}
\newcommand{\mcw}{\mathchanc{w}}
\newcommand{\mcx}{\mathchanc{x}}
\newcommand{\mcy}{\mathchanc{y}}
\newcommand{\mcz}{\mathchanc{z}}



\newcommand{\ba}{\mathbb{a}}
\newcommand{\bb}{\mathbb{b}}
\newcommand{\bc}{\mathbb{c}}
\newcommand{\bd}{\mathbb{d}}
\newcommand{\bg}{\mathbb{g}}
\newcommand{\bh}{\mathbb{h}}
\newcommand{\bi}{\mathbb{i}}
\newcommand{\bj}{\mathbb{j}}
\newcommand{\bk}{\mathbb{k}}
\newcommand{\bl}{\mathbb{l}}
\newcommand{\bm}{\mathbb{m}}
\newcommand{\bn}{\mathbb{n}}
\newcommand{\bo}{\mathbb{o}}
\newcommand{\bp}{\mathbb{p}}
\newcommand{\bq}{\mathbb{q}}
\newcommand{\br}{\mathbb{r}}
\newcommand{\bs}{\mathbb{s}}
\newcommand{\bt}{\mathbb{t}}
\newcommand{\bu}{\mathbb{u}}
\newcommand{\bv}{\mathbb{v}}
\newcommand{\bw}{\mathbb{w}}
\newcommand{\bx}{\mathbb{x}}
\newcommand{\by}{\mathbb{y}}
\newcommand{\bz}{\mathbb{z}}


\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\scr}{\mathcal}
\newcommand{\sA}{\scr{A}}
\newcommand{\sB}{\scr{B}}
\newcommand{\sC}{\scr{C}}
\newcommand{\sD}{\scr{D}}
\newcommand{\sE}{\scr{E}}
\newcommand{\sF}{\scr{F}}
\newcommand{\sG}{\scr{G}}
\newcommand{\sH}{\scr{H}}
\newcommand{\sI}{\scr{I}}
\newcommand{\sJ}{\scr{J}}
\newcommand{\sK}{\scr{K}}
\newcommand{\sL}{\scr{L}}
\newcommand{\sM}{\scr{M}}
\newcommand{\sN}{\scr{N}}
\newcommand{\sO}{\scr{O}}
\newcommand{\sP}{\scr{P}}
\newcommand{\sQ}{\scr{Q}}
\newcommand{\sR}{\scr{R}}
\newcommand{\sS}{\scr{S}}
\newcommand{\sT}{\scr{T}}
\newcommand{\sU}{\scr{U}}
\newcommand{\sV}{\scr{V}}
\newcommand{\sW}{\scr{W}}
\newcommand{\sX}{\scr{X}}
\newcommand{\sY}{\scr{Y}}
\newcommand{\sZ}{\scr{Z}}

\newcommand{\ta}{\widetilde{a}}
\newcommand{\tb}{\widetilde{b}}
\newcommand{\tc}{\widetilde{c}}
\newcommand{\td}{\widetilde{d}}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\tg}{\widetilde{g}}
\newcommand{\ti}{\widetilde{i}}
\newcommand{\tj}{\widetilde{j}}
\newcommand{\tk}{\widetilde{k}}
\newcommand{\tl}{\widetilde{l}}
\newcommand{\tm}{\widetilde{m}}
\newcommand{\tn}{\widetilde{n}}
\newcommand{\tp}{\widetilde{p}}
\newcommand{\tq}{\widetilde{q}}
\newcommand{\ts}{\widetilde{s}}
\newcommand{\tu}{\widetilde{u}}
\newcommand{\tv}{\widetilde{v}}
\newcommand{\tw}{\widetilde{w}}
\newcommand{\tx}{\widetilde{x}}
\newcommand{\ty}{\widetilde{y}}
\newcommand{\tz}{\widetilde{z}}

\newcommand{\tA}{\widetilde{A}}
\newcommand{\tB}{\widetilde{B}}
\newcommand{\tC}{\widetilde{C}}
\newcommand{\tD}{\widetilde{D}}
\newcommand{\tE}{\widetilde{E}}
\newcommand{\tF}{\widetilde{F}}
\newcommand{\tG}{\widetilde{G}}
\newcommand{\tH}{\widetilde{H}}
\newcommand{\tI}{\widetilde{I}}
\newcommand{\tJ}{\widetilde{J}}
\newcommand{\tK}{\widetilde{K}}
\newcommand{\tL}{\widetilde{L}}
\newcommand{\tM}{\widetilde{M}}
\newcommand{\tN}{\widetilde{N}}
\newcommand{\tO}{\widetilde{O}}
\newcommand{\tP}{\widetilde{P}}
\newcommand{\tQ}{\widetilde{Q}}
\newcommand{\tR}{\widetilde{R}}
\newcommand{\tS}{\widetilde{S}}
\newcommand{\tT}{\widetilde{T}}
\newcommand{\tU}{\widetilde{U}}
\newcommand{\tV}{\widetilde{V}}
\newcommand{\tW}{\widetilde{W}}
\newcommand{\tX}{\widetilde{X}}
\newcommand{\tY}{\widetilde{Y}}
\newcommand{\tZ}{\widetilde{Z}}


\newcommand{\oa}{\overline{a}}
\newcommand{\oc}{\overline{c}}
\newcommand{\of}{\overline{f}}
%\newcommand{\og}{\overline{g}}
\newcommand{\oh}{\overline{h}}
\newcommand{\oi}{\overline{i}}
\newcommand{\oj}{\overline{j}}
\newcommand{\ok}{\overline{k}}
\newcommand{\on}{\overline{n}}
\newcommand{\oo}{\overline{o}}
\newcommand{\op}{\overline{p}}
\newcommand{\oq}{\overline{q}}
\newcommand{\os}{\overline{s}}
\newcommand{\ot}{\overline{t}}
\newcommand{\ou}{\overline{u}}
\newcommand{\ov}{\overline{v}}
\newcommand{\ow}{\overline{w}}
\newcommand{\ox}{\overline{x}}
\newcommand{\oy}{\overline{y}}
\newcommand{\oz}{\overline{z}}
\newcommand{\oA}{\overline{A}}
\newcommand{\oB}{\overline{B}}
\newcommand{\oC}{\overline{C}}
\newcommand{\oD}{\overline{D}}
\newcommand{\oE}{\overline{E}}
\newcommand{\oF}{\overline{F}}
\newcommand{\oG}{\overline{G}}
\newcommand{\oH}{\overline{H}}
\newcommand{\oI}{\overline{I}}
\newcommand{\oJ}{\overline{J}}
\newcommand{\oK}{\overline{K}}
\newcommand{\oL}{\overline{L}}
\newcommand{\oM}{\overline{M}}
\newcommand{\oN}{\overline{N}}
\newcommand{\oO}{\overline{O}}
\newcommand{\oP}{\overline{P}}
\newcommand{\oQ}{\overline{Q}}
\newcommand{\oR}{\overline{R}}
\newcommand{\oS}{\overline{S}}
\newcommand{\oT}{\overline{T}}
\newcommand{\oU}{\overline{U}}
\newcommand{\oV}{\overline{V}}
\newcommand{\oW}{\overline{W}}
\newcommand{\oX}{\overline{X}}
\newcommand{\oY}{\overline{Y}}
\newcommand{\oZ}{\overline{Z}}

\DeclareMathOperator{\Bij}{{Bij}}
\DeclareMathOperator{\characteristic}{{Char}}
\DeclareMathOperator{\SB}{{\mathbf{SB}}}
\DeclareMathOperator{\nt}{{nt}}
\DeclareMathOperator{\alg}{{alg}}
\DeclareMathOperator{\discrep}{{discrep}}
\DeclareMathOperator{\Art}{{Art}}
\DeclareMathOperator{\trdeg}{{trdeg}}
\DeclareMathOperator{\mld}{{mld}}
\DeclareMathOperator{\lct}{{lct}}
\DeclareMathOperator{\Bs}{{Bs}}
\DeclareMathOperator{\Fix}{{Fix}}
\DeclareMathOperator{\Bir}{{Bir}}
\DeclareMathOperator{\rad}{{rad}}
\DeclareMathOperator{\nilp}{{nilp}}
\DeclareMathOperator{\Rad}{{Rad}}
\DeclareMathOperator{\qc}{{qc}}
\DeclareMathOperator{\ch}{{ch}}
\DeclareMathOperator{\todd}{{td}}
\DeclareMathOperator{\nil}{{nil}}
\DeclareMathOperator{\Gor}{{Gor}}
\DeclareMathOperator{\Nil}{{Nil}}
\DeclareMathOperator{\tors}{{tors}}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\Ric}{Ric}
\DeclareMathOperator{\reldim}{{reldim}}
\DeclareMathOperator{\ks}{{ks}}
\DeclareMathOperator{\ind}{{ind}}
\DeclareMathOperator{\iks}{{iks}}
\DeclareMathOperator{\tr}{{tr}}
\DeclareMathOperator{\ev}{{ev}}
\DeclareMathOperator{\cond}{{cond}}
\DeclareMathOperator{\Prod}{{Prod}}
\DeclareMathOperator{\can}{{can}}
\DeclareMathOperator{\sstab}{{ss}}
\DeclareMathOperator{\alb}{{alb}}
\DeclareMathOperator{\Alb}{{Alb}}
\DeclareMathOperator{\Sym}{{Sym}}
\DeclareMathOperator{\aut}{{Aut}}
\DeclareMathOperator{\lcm}{{lcm}}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Ann}{\mcA\mcn\mcn}
\DeclareMathOperator{\ann}{\mca\mcn\mcn}
\DeclareMathOperator{\bir}{{Bir}}
\DeclareMathOperator{\Bl}{{Bl}}
\DeclareMathOperator{\charact}{char}
\DeclareMathOperator{\Chow}{Chow}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\coker}{{coker}}
\DeclareMathOperator{\Gal}{{Gal}}
\DeclareMathOperator{\Ker}{{Ker}}
\DeclareMathOperator{\pre}{{pre}}
\DeclareMathOperator{\adj}{{adj}}
\DeclareMathOperator{\depth}{{depth}} 
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\diff}{Diff}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\opdiv}{div}
\DeclareMathOperator{\Dubbies}{Dubbies^n}
%
\DeclareMathOperator{\Ex}{Ex}
\DeclareMathOperator{\exc}{exc}
\DeclareMathOperator{\Exc}{Exc}
\DeclareMathOperator{\fpt}{fpt}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\ext}{{Ext}}
\newcommand{\sExt}[0]{{\mcE\mcx\mct}}    
\DeclareMathOperator{\gl}{{GL}}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\Fam}{Fam}
\DeclareMathOperator{\rref}{rref}
\DeclareMathOperator{\Gr}{{Gr}}
\DeclareMathOperator{\Hilb}{Hilb}
%\DeclareMathOperator{\hom}{{Hom}}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Tor}{Tor}
\newcommand{\sHom}[0]{{\mcH\mco\mcm}}    
\newcommand{\sEnd}[0]{{\mcE\mcn\mcd}}    
\newcommand{\Set}[0]{{\mathfrak{Set}}}    
\newcommand{\Grp}[0]{{\mathfrak{Grp}}}    
\newcommand{\sDer}[0]{{\mcD\mce\mcr}}    
\newcommand{\sRHom}[0]{{\mcR\mcH\mco\mcm}}    
\newcommand{\sTor}[0]{{\mcT\mco\mcr}}    
%\DeclareMathOperator{\Hombir}{Hom_{bir}^n}
\DeclareMathOperator{\id}{{id}}
\DeclareMathOperator{\Id}{{Id}}
\DeclareMathOperator{\im}{{im}}
\DeclareMathOperator{\irr}{{irr}}
\DeclareMathOperator{\Image}{Image}
%\DeclareMathOperator{\Im}{Im}
\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\Jac}{{Jac}}
%\DeclareMathOperator{\ker}{{ker}}
\DeclareMathOperator{\lc}{lc}
\DeclareMathOperator{\length}{{length}}
\DeclareMathOperator{\lin}{{Lin}}
\DeclareMathOperator{\tot}{{tot}}
\DeclareMathOperator{\Locus}{Locus}
\DeclareMathOperator{\mor}{{Mor}}
\DeclareMathOperator{\Mor}{{Mor}}
\DeclareMathOperator{\mult}{mult} 
\DeclareMathOperator{\stab}{stab} 
\DeclareMathOperator{\Num}{Num}
\DeclareMathOperator{\ord}{{ord}}
\DeclareMathOperator{\rel}{{rel}}
\DeclareMathOperator{\Ob}{{Ob}}
\DeclareMathOperator{\ob}{{Ob}}
\DeclareMathOperator{\pic}{{Pic}}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Weil}{Weil}
\DeclareMathOperator{\APic}{APic}
\DeclareMathOperator{\pico}{{Pic}^{\circ}}
\DeclareMathOperator{\pgl}{{PGL}}
\DeclareMathOperator{\PGL}{{PGL}}
\DeclareMathOperator{\GL}{{GL}}
\DeclareMathOperator{\Mat}{{Mat}}
\DeclareMathOperator{\psl}{PSL} 
\DeclareMathOperator{\PSL}{PSL} 
\DeclareMathOperator{\Proj}{{Proj}}
\DeclareMathOperator{\ptRC}{{RC_{\bullet}}}
\DeclareMathOperator{\ptUnivrc}{{Univ^{rc}_{\bullet}}}
\DeclareMathOperator{\RatCurves}{RatCurves^n}
\DeclareMathOperator{\rank}{{rank}}
\DeclareMathOperator{\RC}{RatCurves^n}
\DeclareMathOperator{\NE}{{\overline{NE}}}
\DeclareMathOperator{\pt}{pt}
\DeclareMathOperator{\pts}{pts}
\newcommand{\homstack}{\underline{\sHom}}
%
\DeclareMathOperator{\red}{red}
\DeclareMathOperator{\Reg}{Reg}
\DeclareMathOperator{\Eff}{Eff}
\DeclareMathOperator{\reg}{reg}
\DeclareMathOperator{\sing}{sing}
\DeclareMathOperator{\sm}{sm}
\DeclareMathOperator{\rtl}{rtl}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\wst}{wst}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\rk}{{rk}}
\DeclareMathOperator{\Sing}{{Sing}}
\DeclareMathOperator{\sgn}{{sgn}}
\DeclareMathOperator{\Spec}{{Spec}}
\DeclareMathOperator{\coeff}{{coeff}}
\DeclareMathOperator{\supp}{{supp}}
\DeclareMathOperator{\fppf}{{fppf}}
\DeclareMathOperator{\Supp}{{Supp}}
\DeclareMathOperator{\Stab}{{Stab}}
\DeclareMathOperator{\sym}{{Sym}}
\DeclareMathOperator{\twoRC}{{RC_2^n}}
\DeclareMathOperator{\twoptRC}{{RC^2_{\bullet}}}
\DeclareMathOperator{\twoUnivrc}{{Univ^{rc, 2}}}
\DeclareMathOperator{\twoptUnivrc}{{Univ_{\bullet}^{rc, 2}}}
\DeclareMathOperator{\Univ}{Univ}
\DeclareMathOperator{\Univrc}{{Univ^{rc}}}
\DeclareMathOperator{\var}{{Var}}
\DeclareMathOperator{\Var}{{Var}}
\DeclareMathOperator{\CaCl}{{CaCl}}
\DeclareMathOperator{\Ca}{{Ca}}
\DeclareMathOperator{\disc}{{disc}}
\DeclareMathOperator{\hocolim}{\underset{\longrightarrow}{hocolim}}
\DeclareMathOperator{\holim}{\underset{\longleftarrow}{holim}}
\DeclareMathOperator{\Nklt}{Nklt}

\newcommand{\factor}[2]{\left. \raise 2pt\hbox{\ensuremath{#1}} \right/
        \hskip -2pt\raise -2pt\hbox{\ensuremath{#2}}}

\renewcommand{\theequation}{\arabic{section}.\arabic{subsection}.\arabic{theorem}.\alph{equation}}

%\counterwithin*{equation}{section}
%\counterwithin*{equation}{subsection}
%\counterwithin*{equation}{theorem}
%\counterwithin*{equation}{proof}

\makeatletter
\renewcommand\subsection{
  \renewcommand{\sfdefault}{pag}
  \@startsection{subsection}%
  {2}{0pt}{.8\baselineskip}{.4\baselineskip}{\raggedright
    \sffamily\itshape\small\bfseries
  }}
\renewcommand\section{
  \renewcommand{\sfdefault}{phv}
  \@startsection{section} %
  {1}{0pt}{\baselineskip}{.8\baselineskip}{\centering
    \sffamily
    \scshape
    \bfseries
}}
\makeatother

%\renewcommand{\theenumi}{\arabic{enumi}}

\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}

\newcommand{\ofA}{\overline{\mathfrak{A}}}
\newcommand{\ofB}{\overline{\mathfrak{B}}}
\newcommand{\ofC}{\overline{\mathfrak{C}}}
\newcommand{\ofD}{\overline{\mathfrak{D}}}
\newcommand{\ofE}{\overline{\mathfrak{E}}}
\newcommand{\ofF}{\overline{\mathfrak{F}}}
\newcommand{\ofG}{\overline{\mathfrak{G}}}
\newcommand{\ofH}{\overline{\mathfrak{H}}}
\newcommand{\ofI}{\overline{\mathfrak{I}}}
\newcommand{\ofJ}{\overline{\mathfrak{J}}}
\newcommand{\ofK}{\overline{\mathfrak{K}}}
\newcommand{\ofL}{\overline{\mathfrak{L}}}
\newcommand{\ofM}{\overline{\mathfrak{M}}}
\newcommand{\ofN}{\overline{\mathfrak{N}}}
\newcommand{\ofO}{\overline{\mathfrak{O}}}
\newcommand{\ofP}{\overline{\mathfrak{P}}}
\newcommand{\ofQ}{\overline{\mathfrak{Q}}}
\newcommand{\ofR}{\overline{\mathfrak{R}}}
\newcommand{\ofS}{\overline{\mathfrak{S}}}
\newcommand{\ofT}{\overline{\mathfrak{T}}}
\newcommand{\ofU}{\overline{\mathfrak{U}}}
\newcommand{\ofV}{\overline{\mathfrak{V}}}
\newcommand{\ofW}{\overline{\mathfrak{W}}}
\newcommand{\ofX}{\overline{\mathfrak{X}}}
\newcommand{\ofY}{\overline{\mathfrak{Y}}}
\newcommand{\ofZ}{\overline{\mathfrak{Z}}}

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}\newcommand{\osa}{\overline{\scr{a}}}

\newcommand{\osb}{\overline{\scr{b}}}
\newcommand{\osc}{\overline{\scr{c}}}
\newcommand{\osd}{\overline{\scr{d}}}
\newcommand{\ose}{\overline{\scr{e}}}
\newcommand{\osf}{\overline{\scr{f}}}
\newcommand{\osg}{\overline{\scr{g}}}
\newcommand{\osh}{\overline{\scr{h}}}
\newcommand{\osi}{\overline{\scr{i}}}
\newcommand{\osj}{\overline{\scr{j}}}
\newcommand{\osk}{\overline{\scr{k}}}
\newcommand{\osl}{\overline{\scr{l}}}
\newcommand{\osm}{\overline{\scr{m}}}
\newcommand{\osn}{\overline{\scr{n}}}
\newcommand{\oso}{\overline{\scr{o}}}
\newcommand{\osp}{\overline{\scr{p}}}
\newcommand{\osq}{\overline{\scr{q}}}
\newcommand{\osr}{\overline{\scr{r}}}
\newcommand{\oss}{\overline{\scr{s}}}
\newcommand{\ost}{\overline{\scr{t}}}
\newcommand{\osu}{\overline{\scr{u}}}
\newcommand{\osv}{\overline{\scr{v}}}
\newcommand{\osw}{\overline{\scr{w}}}
\newcommand{\osx}{\overline{\scr{x}}}
\newcommand{\osy}{\overline{\scr{y}}}
\newcommand{\osz}{\overline{\scr{z}}}
\newcommand{\osA}{\overline{\scr{A}}}
\newcommand{\osB}{\overline{\scr{B}}}
\newcommand{\osC}{\overline{\scr{C}}}
\newcommand{\osD}{\overline{\scr{D}}}
\newcommand{\osE}{\overline{\scr{E}}}
\newcommand{\osF}{\overline{\scr{F}}}
\newcommand{\osG}{\overline{\scr{G}}}
\newcommand{\osH}{\overline{\scr{H}}}
\newcommand{\osI}{\overline{\scr{I}}}
\newcommand{\osJ}{\overline{\scr{J}}}
\newcommand{\osK}{\overline{\scr{K}}}
\newcommand{\osL}{\overline{\scr{L}}}
\newcommand{\osM}{\overline{\scr{M}}}
\newcommand{\osN}{\overline{\scr{N}}}
\newcommand{\osO}{\overline{\scr{O}}}
\newcommand{\osP}{\overline{\scr{P}}}
\newcommand{\osQ}{\overline{\scr{Q}}}
\newcommand{\osR}{\overline{\scr{R}}}
\newcommand{\osS}{\overline{\scr{S}}}
\newcommand{\osT}{\overline{\scr{T}}}
\newcommand{\osU}{\overline{\scr{U}}}
\newcommand{\osV}{\overline{\scr{V}}}
\newcommand{\osW}{\overline{\scr{W}}}
\newcommand{\osX}{\overline{\scr{X}}}
\newcommand{\osY}{\overline{\scr{Y}}}
\newcommand{\osZ}{\overline{\scr{Z}}}

\setcounter{tocdepth}{2}

\newcommand{\oba}{\overline{\mathbb{a}}}
\newcommand{\obb}{\overline{\mathbb{b}}}
\newcommand{\obc}{\overline{\mathbb{c}}}
\newcommand{\obd}{\overline{\mathbb{d}}}
\newcommand{\obe}{\overline{\mathbb{e}}}
\newcommand{\obf}{\overline{\mathbb{f}}}
\newcommand{\obg}{\overline{\mathbb{g}}}
\newcommand{\obh}{\overline{\mathbb{h}}}
\newcommand{\obi}{\overline{\mathbb{i}}}
\newcommand{\obj}{\overline{\mathbb{j}}}
\newcommand{\obk}{\overline{\mathbb{k}}}
\newcommand{\obl}{\overline{\mathbb{l}}}
\newcommand{\obm}{\overline{\mathbb{m}}}
\newcommand{\obn}{\overline{\mathbb{n}}}
\newcommand{\obo}{\overline{\mathbb{o}}}
\newcommand{\obp}{\overline{\mathbb{p}}}
\newcommand{\obq}{\overline{\mathbb{q}}}
\newcommand{\obr}{\overline{\mathbb{r}}}
\newcommand{\obs}{\overline{\mathbb{s}}}
\newcommand{\obt}{\overline{\mathbb{t}}}
\newcommand{\obu}{\overline{\mathbb{u}}}
\newcommand{\obv}{\overline{\mathbb{v}}}
\newcommand{\obw}{\overline{\mathbb{w}}}
\newcommand{\obx}{\overline{\mathbb{x}}}
\newcommand{\oby}{\overline{\mathbb{y}}}
\newcommand{\obz}{\overline{\mathbb{z}}}
\newcommand{\obA}{\overline{\mathbb{A}}}
\newcommand{\obB}{\overline{\mathbb{B}}}
\newcommand{\obC}{\overline{\mathbb{C}}}
\newcommand{\obD}{\overline{\mathbb{D}}}
\newcommand{\obE}{\overline{\mathbb{E}}}
\newcommand{\obF}{\overline{\mathbb{F}}}
\newcommand{\obG}{\overline{\mathbb{G}}}
\newcommand{\obH}{\overline{\mathbb{H}}}
\newcommand{\obI}{\overline{\mathbb{I}}}
\newcommand{\obJ}{\overline{\mathbb{J}}}
\newcommand{\obK}{\overline{\mathbb{K}}}
\newcommand{\obL}{\overline{\mathbb{L}}}
\newcommand{\obM}{\overline{\mathbb{M}}}
\newcommand{\obN}{\overline{\mathbb{N}}}
\newcommand{\obO}{\overline{\mathbb{O}}}
\newcommand{\obP}{\overline{\mathbb{P}}}
\newcommand{\obQ}{\overline{\mathbb{Q}}}
\newcommand{\obR}{\overline{\mathbb{R}}}
\newcommand{\obS}{\overline{\mathbb{S}}}
\newcommand{\obT}{\overline{\mathbb{T}}}
\newcommand{\obU}{\overline{\mathbb{U}}}
\newcommand{\obV}{\overline{\mathbb{V}}}
\newcommand{\obW}{\overline{\mathbb{W}}}
\newcommand{\obX}{\overline{\mathbb{X}}}
\newcommand{\obY}{\overline{\mathbb{Y}}}
\newcommand{\obZ}{\overline{\mathbb{Z}}}

